Explainable AI Systems Must Be Contestable: Here's How to Make It Happen

As AI regulations around the world intensify their focus on system safety, contestability has become a mandatory, yet ill-defined, safeguard. In XAI, "contestability" remains an empty promise: no formal definition exists, no algorithm guarantees it, and practitioners lack concrete guidance to satisfy regulatory requirements. Grounded in a systematic literature review, this paper presents the first rigorous formal definition of contestability in explainable AI, directly aligned with stakeholder requirements and regulatory mandates. We introduce a modular framework of by-design and post-hoc mechanisms spanning human-centered interfaces, technical architectures, legal processes, and organizational workflows. To operationalize our framework, we propose the Contestability Assessment Scale, a composite metric built on more than twenty quantitative criteria. Through multiple case studies across diverse application domains, we reveal where state-of-the-art systems fall short and show how our framework drives targeted improvements. By converting contestability from regulatory theory into a practical framework, our work equips practitioners with the tools to embed genuine recourse and accountability into AI systems.

==> tables/tab_dimensions_color.tex <==

\begin{table}[ht]
\centering
\caption{Dimension Tags for Contestability}
\label{tab:dimension-tags}
\begin{tabularx}{\linewidth}{@{}>{\hspace{0pt}}lX@{}}
\toprule
\textbf{Tag} & \textbf{Definition} \\
\midrule
\rowcolor{lightgray} \footnotesize
\textbf{Human-Centered} & \footnotesize
Design and evaluation criteria that prioritize the experiences, needs, and rights of individuals and communities affected by AI systems. These dimensions emphasize usability, inclusivity, emotional well-being, cultural adaptation, and participatory design, drawing from HCI, cognitive ergonomics, and user-centered ethics. \\
\footnotesize
\textbf{Technical} & \footnotesize
Computational, architectural, and algorithmic properties that enable contestability. Includes logging, explainability mechanisms, real-time overrides, system security, and data management. Grounded in software engineering, computer security, and XAI literature. \\
\rowcolor{lightgray}
\footnotesize
\textbf{Legal} & \footnotesize
Normative, statutory, and regulatory requirements that guarantee contestability as a right. Reflects due process, privacy protection, transparency obligations (e.g., GDPR), and legal enforceability of redress. Informed by data protection law, administrative law, and AI ethics regulations. \\
\footnotesize
\textbf{Organizational} & \footnotesize
Institutional structures, accountability protocols, and governance practices that embed contestability across the AI lifecycle. Includes role assignments, escalation workflows, transparency reporting, and learning from feedback. Draws on institutional theory, risk management, and sociotechnical systems design. \\
\bottomrule
\end{tabularx}
\end{table}


==> tables/tab_dimensions_nocolor.tex <==


\begin{table}[ht]
\centering
\caption{Dimension Tags for Contestability}
\begin{tabularx}{\linewidth}{@{}lX@{}}
\toprule
\textbf{Tag} & \textbf{Definition} \\ 
\midrule
\textbf{Human-Centered} & 
Design and evaluation criteria that prioritize the experiences, needs, and rights of individuals and communities affected by AI systems. These dimensions emphasize usability, inclusivity, emotional well-being, cultural adaptation, and participatory design, drawing from HCI, cognitive ergonomics, and user-centered ethics. \\
\addlinespace
\textbf{Technical} & 
Computational, architectural, and algorithmic properties that enable contestability. Includes logging, explainability mechanisms, real-time overrides, system security, and data management. Grounded in software engineering, computer security, and XAI literature. \\
\addlinespace
\textbf{Legal} & 
Normative, statutory, and regulatory requirements that guarantee contestability as a right. Reflects due process, privacy protection, transparency obligations (e.g., GDPR), and legal enforceability of redress. Informed by data protection law, administrative law, and AI ethics regulations. \\
\addlinespace
\textbf{Organizational} & 
Institutional structures, accountability protocols, and governance practices that embed contestability across the AI lifecycle. Includes role assignments, escalation workflows, transparency reporting, and learning from feedback. Draws on institutional theory, risk management, and sociotechnical systems design. \\
\bottomrule
\end{tabularx}
\end{table}


==> tables/tab_framework.tex <==

\begin{table*}[ht]
\footnotesize
\caption{Contestability Levels by AI Reliance}
\begin{tabularx}{\linewidth}{>{\raggedright\arraybackslash}p{3.5cm}X X X}
\toprule
\textbf{Level / Reliance} & \textbf{Low} & \textbf{Medium} & \textbf{High} \\
\midrule

\textbf{Basic} &
\textbf{Necessary:} \newline
 Accessibility \& Resource Equity \taghuman \newline
 Multichannel Access and Advocacy \taghuman \newline
 Education and Right-to-Know (Legal) \newline
 Cultural and Linguistic Adaptation \taghuman 
& 
\textbf{Necessary (+Process Integrity):} \newline
– Explainability–Recourse Coupling (Tech) \newline
– Granular Contestability (Tech) \newline
– Actionability and Outcome Influence (Legal) \newline
– Real-Time Contestation for Critical Systems (Tech) \newline
– Non-Retaliation Guarantee (Legal)
& 
\textbf{Necessary (+Governance):} \newline
– Traceability and Audit Logging (Tech) \newline
– Regulatory Auditability and Public Oversight (Legal) \newline
– Assigned Responsibility \& Escalation Paths (Org) \newline
– Clarity on Contestability Boundaries (Legal) 
\\

\textbf{Intermediate} &
\textbf{Necessary (Process Integrity):} \newline
– Explainability–Recourse Coupling (Tech) \newline
– Granular Contestability (Tech) \newline
– Actionability and Outcome Influence (Legal) \newline
– Real-Time Contestation (Tech) \newline
– Non-Retaliation Guarantee (Legal)
& 
\textbf{Necessary:} \newline
– Traceability and Audit Logging (Tech) \newline
– Regulatory Auditability and Public Oversight (Legal) \newline
– Assigned Responsibility \& Escalation Paths (Org) \newline
– Clarity on Contestability Boundaries (Legal)
& 
\textbf{Necessary:} \newline
– Systemic Learning from Contestation Data (Org) \newline
– Continuous Monitoring of Contestation Barriers (Org) \newline
– Stakeholder Co-Design \& Participatory Development \taghuman \newline
– Context Sensitivity \& Risk Scaling (Tech) \newline
– Outcome Impact Assessment \taghuman 
\\

\textbf{Advanced} &
\textbf{Necessary (Governance):} \newline
– Traceability and Audit Logging (Tech) \newline
– Regulatory Auditability and Public Oversight (Legal) \newline
– Assigned Responsibility \& Escalation Paths (Org) \newline
– Clarity on Contestability Boundaries (Legal)
& 
\textbf{Necessary (+Adaptation):} \newline
– Systemic Learning from Contestation Data (Org) \newline
– Continuous Monitoring of Contestation Barriers (Org) \newline
– Stakeholder Co-Design \& Participatory Development (\taghuman) \newline
– Context Sensitivity \& Risk Scaling (Tech) \newline
– Outcome Impact Assessment (\taghuman)
& 
\textbf{Necessary (+Supportive):} \newline
– Privacy-Preserving Contestation (Tech) \newline
– Technological Robustness \& Security (Tech) \newline
– Psychological Safety \& Emotional Support (\taghuman) \newline
– Transparency of Contestation Outcomes (Org)
\\
\bottomrule
\end{tabularx}
\end{table*}

